CF-GNNExplainer: Counterfactual Explanations for Graph Neural Networks

Given the increasing promise of graph neural networks (GNNs) in real-world applications, several methods have been developed for explaining their predictions. Existing methods for interpreting predictions from GNNs have primarily focused on generating subgraphs that are especially relevant for a particular prediction. However, such methods are not counterfactual (CF) in nature: given a prediction, we want to understand how the prediction can be changed in order to achieve an alternative outcome. In this work, we propose a method for generating CF explanations for GNNs: the minimal perturbation to the input (graph) data such that the prediction changes. Using only edge deletions, we find that our method, CF-GNNExplainer, can generate CF explanations for the majority of instances across three widely used datasets for GNN explanations, while removing less than 3 edges on average, with at least 94\% accuracy. This indicates that CF-GNNExplainer primarily removes edges that are crucial for the original predictions, resulting in minimal CF explanations.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{section:introduction}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Sections~\ref{section:datasets}, \ref{section:complexity}, \ref{section:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{section:limitations}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{This work does not include any Theorems.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{This work does not include any Theorems.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We included the code and datasets in the Supplementary Material..}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, see Section~\ref{section:experimental-setup}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Our method is deterministic and therefore changing the random seed does not have an influence on the results, since we always initialize $\perturbb$ as a matrix of 1s. We double-checked to make sure, and indeed, after trying 5 different random seeds per experiment, the results were exactly the same every time.} 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{section:experimental-setup}. 
    % The method we develop does not require a huge amount of resources, indeed.
    }
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{section:experimental-setup}.}
  \item Did you mention the license of the assets?
    \answerNA{We only use materials from public GitHub repositories.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{All code and datasets are available in the Supplementary Material. }
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We are not using data from people in our study.}  
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We did not conduct research with human subjects. } 
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/results-v2.tex <==
%!TEX root = ../main.tex

\begin{table*}[h]
\centering
\caption{Results comparing our method (denoted \OurShort{}) to \baserand{}, \basekeep{}, and \baserm{}. Below each metric, $\blacktriangledown$ indicates a low value is desirable, while $\blacktriangle$ indicates a high value is desirable.}
\label{table:results}
\setlength{\tabcolsep}{4pt}
%\footnotesize{
\begin{tabular}{lrrrr rrrr rrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\synfour{}}                                                                                                                 & \multicolumn{4}{c}{\synfive{}}                                                                                                                   & \multicolumn{4}{c}{\synone{}}                                                                                                                  \\ 
\cmidrule(r){2-5}\cmidrule(r){6-9}\cmidrule{10-13} 
               & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Size}} & \multicolumn{1}{c}{\textit{Spars.}} & \multicolumn{1}{c}{\textit{Acc.}} & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Size}} & \multicolumn{1}{c}{\textit{Spars.}} & \multicolumn{1}{c}{\textit{Acc.}} & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Size}} & \multicolumn{1}{c}{\textit{Spars.}} & \multicolumn{1}{c}{\textit{Acc.}} \\

% & \multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\uparrow$} \\

Method & \multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangle$} \\
\midrule
\baserand{}               & \textbf{0.00}                     & 4.70                              & 0.79                                & 0.63                               & \textbf{0.00}                     & 9.06                              & 0.75                                & 0.77                               & \textbf{0.00}                     & 503.31                            & 0.58                                & 0.17                              \\
\basekeep{}                 & 0.32                              & 15.64                             & 0.13                                & 0.45                               & 0.32                              & 29.30                             & 0.09                                & 0.72                               & 0.60                              & 504.18                            & 0.05                                & 0.18                              \\
\baserm{}              & 0.46                              & 2.11                              & 0.89                                & ---                                  & 0.61                              & 2.27                              & 0.92                                & ---                                  & 0.21                              & 10.56                             & 0.97                                & \textbf{0.99}                     \\
\midrule
\OurShort{}               & 0.21                              & \textbf{2.09}                     & \textbf{0.90}                       & \textbf{0.94}                      & 0.07                              & \textbf{1.47}                     & \textbf{0.94}                       & \textbf{0.96}                      & 0.39                              & \textbf{2.39}                     & \textbf{0.99}                       & 0.96                 \\
\bottomrule
\end{tabular}
%}
\end{table*}

\begin{figure*}[]

    \centering

    \includegraphics[scale=0.38]{images/tree-cycles-random.png}
    \includegraphics[scale=0.38]{images/tree-grid-random.png}
    \includegraphics[scale=0.38]{images/ba-shapes-random.png}
    
        \caption{Histograms showing \textit{Explanation Size} from \baserand{}. Note the x-axis for \synone{} goes up to 1500. Left: \synfour{}, Middle: \synfive{}, Right: \synone{}.  }
        \label{fig:random-explanation-size}
        
    \includegraphics[scale=0.38]{images/tree-cycles-keep.png}
    \includegraphics[scale=0.38]{images/tree-grid-keep.png}
    \includegraphics[scale=0.38]{images/ba-shapes-keep.png}
    
        \caption{Histograms showing \textit{Explanation Size} from \basekeep{}. Note the x-axis for \synone{} goes up to 1500. Left: \synfour{}, Middle: \synfive{}, Right: \synone{}. }
        \label{fig:keep-explanation-size}
        
        
    \includegraphics[scale=0.38]{images/tree-cycles-remove.png}
    \includegraphics[scale=0.38]{images/tree-grid-remove.png}
    \includegraphics[scale=0.38]{images/ba-shapes-remove.png}
    
        \caption{Histograms showing \textit{Explanation Size} from \baserm{}. Note the x-axis for \synone{} goes up to 70. Left: \synfour{}, Middle: \synfive{}, Right: \synone{}. }
        \label{fig:remove-explanation-size}
        
    % \includegraphics[scale=0.38]{images/tree-cycles-gnnexplainer.png}
    % \includegraphics[scale=0.38]{images/tree-grid-gnnexplainer.png}
    % \includegraphics[scale=0.38]{images/ba-shapes-gnnexplainer.png}
    
    %     \caption{Histograms showing \textit{Explanation Size} from \gnnexplainer{}. Note that the y-axis goes up to 1. Left: \synfour{}, Middle: \synfive{}, Right: \synone{}.}
    %     \label{fig:gnnexplainer-explanation-size}

    \includegraphics[scale=0.38]{images/tree-cycles.png}
    \includegraphics[scale=0.38]{images/tree-grid.png}
    \includegraphics[scale=0.38]{images/ba-shapes.png}
    
        \caption{Histograms showing \textit{Explanation Size} from \OurMethod{}. Note the x-axis for \synone{} goes up to 70. Left: \synfour{}, Middle: \synfive{}, Right: \synone{}. }
        \label{fig:explanation-size}
        
\end{figure*}









\section{Results}
\label{section:results}
We evaluate \OurMethod{} in terms of the metrics outlined in Section~\ref{section:metrics}. 
The results are shown in Tables~\ref{table:results} and ~\ref{table:results-gnnexplainer}.  
In almost all settings, we find that \OurMethod{} outperforms the baselines in terms of \textit{Explanation Size}, \textit{Subgraph Impact}, and \textit{Accuracy}, which shows that \OurMethod{} satisfies our objective of finding accurate, minimal CF examples. 
In cases where other methods outperform \OurMethod{} on a particular metric, these methods perform poorly on the rest of the metrics, or on other datasets. 





\textbf{Fidelity:}
 \OurMethod{} outperforms \basekeep{} across all three datasets, and outperforms \baserm{} for \synfour{} and \synfive{} in terms of \textit{Fidelity}. 
We find that \baserand{} has the lowest \textit{Fidelity} in all cases -- it is able to find CF examples for every single node. 
In the following subsections, we will see that this corresponds to poor performance on the other metrics.
% , and it does not satisfy our objective of finding accurate, minimal CF examples. 


% Across all three datasets, \OurMethod{} is able to generate CF examples for the majority of instances, but not all of them. 
% We find that \baserand{} has the highest \textit{Coverage} $= 1$ for all three datasets -- it is able to find CF examples for every single node, and therefore outperforms \OurMethod{} for this metric. 
% However, in the following subsections, we will see that this comes at a high cost. \baserand{} performs poorly on the other three metrics, i.e., it does not satisfy our objective of finding accurate, minimal CF examples.



\textbf{Explanation Size:}
Figures~\ref{fig:random-explanation-size} to ~\ref{fig:explanation-size} show histograms of the \textit{Explanation Size} for the five methods we compare.
% \footnote{We remind the reader that the \textit{Explanation Size} for \gnnexplainer{} is equal to the user-input parameter $S$ (see Section~\ref{section:baselines}). It is possible for the \textit{Explanation Size} to be less than $S$ if and only if there are less than $S$ edges in the \cgraph{} of a node $v$. This is possible only for nodes outside of the motifs. However, based on Figure~\ref{fig:gnnexplainer-explanation-size}, we see that this is rarely the case, and that in almost 100\% of cases, \textit{Explanation Size} $= S$.}

We see that across all three datasets, \OurMethod{} has the smallest (i.e., most minimal) \textit{Explanation Sizes}. 
This is especially true when comparing to \baserand{} and \basekeep{} for the \synone{} dataset, where we had to use a different scale for the x-axis due to how different the \textit{Explanation Sizes} were. 
We postulate that this difference could be because \synone{} is a much more densely connected graph;
it has fewer nodes but more edges compared to the other two datasets, and the average number of nodes and edges in the \cgraph{} is order(s) of magnitude larger (see Table~\ref{table:stats}). 
Therefore, when performing random perturbations, there is substantial opportunity to remove edges that do not necessarily need to be removed, leading to much larger \textit{Explanation Sizes}.
When there are many edges in the \cgraph{}, removing everything except the 1-hop neighbourhood, as is done in \basekeep{}, also results in large \textit{Explanation Sizes}. 
In contrast, the loss function used by \OurMethod{} ensures that only a few edges are removed, which is the desirable behavior since we want minimal explanations. 




% We see that for \synfour{} and \synfive{}, that the majority of CF examples, around 60\%, are created by removing only one edge from the original generated subgraph (i.e., \textit{Explanation Size} = 1). 
% The \synone{} histogram is much flatter in comparison, with the majority of CF examples having\textit{ Explanation Size} = 3. 
% \synone{} also has a higher mean \textit{Explanation Size} = 2.24 compared to 1.78 for \synfour{} and 1.47 for \synfive{} (see Table~\ref{table:results}). 
% We postulate that this difference could be because \synone{} is a much more densely connected graph;
% it has less nodes but more edges compared to the other two datasets (see Table~\ref{table:stats}). 
% Moreover, its average node degree is more than double that of the other two datasets. 
% This could be why its CF examples have larger \textit{Explanation Sizes}. 




\textbf{Sparsity:}
\OurMethod{} outperforms all four baselines for all three datasets in terms of \textit{Sparsity}. 
We note \OurMethod{} and \baserm{} perform much better on this metric in comparison to the other methods, which aligns with the results from \textit{Explanation Size}. 
% since these two metrics are inherently related.  

% For \OurMethod{} and \baserand{}, we see that \synone{} has the lowest \textit{Subgraph Impact} out of the three datasets. 
% This is most likely because each $\compadj$ in \synone{} has many more edges compared to \synfour{} or \synfive{}: on average, the number of edges in each $\compadj$ in \synone{} is two orders of magnitude larger than for the other two datasets (see Table~\ref{table:stats}). 
% This means that the denominator we use is much larger, resulting in a smaller value for \textit{Subgraph Impact}. 
% We also note that across all three datasets, in agreement with  our objective, the \textit{Subgraph Impact} is low for \OurMethod{}: in the worst case (\synfour{}), we are removing 12\% of edges, while in the best case (\synone{}), we are removing less than 1\% of edges in $\compadj$ (see Table~\ref{table:results}).

%We outperform \baserand{} in terms of \textit{Subgraph Impact} for all three datasets. 

\textbf{Accuracy:}
We observe that \OurMethod{} has the highest \textit{Accuracy} for the \synfour{} and \synfive{} datasets, whereas \baserm{} has the highest \textit{Accuracy} for \synone{}. 
However, we are unable to calculate the accuracy of \baserm{} for the other two datasets since it is unable to generate \emph{any} CF examples for motif nodes, contributing to the low \textit{Coverage} on those datasets. 
We observe \textit{Accuracy} levels upwards of 94\% for \OurMethod{} across \emph{all} datasets, indicating that it is consistent in correctly removes edges that are crucial for the initial predictions in the vast majority of cases (see Table~\ref{table:results}). 












\begin{table*}[]
\centering
\caption{Results comparing our method (denoted \OurShort{}) to \gnnexplainer{}, for varying values of S. \OurShort{} finds S automatically. Below each metric, $\blacktriangledown$ indicates a low value is desirable, while $\blacktriangle$ indicates a high value is desirable.}
\label{table:results-gnnexplainer}
\setlength{\tabcolsep}{4pt}
%\footnotesize{
\begin{tabular}{lrrrr rrrr rrrr}
\toprule
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\synfour{}}                                                                                                                 & \multicolumn{4}{c}{\synfive{}}                                                                                                                   & \multicolumn{4}{c}{\synone{}}                                                                                                                  \\ 
\cmidrule(r){2-5}\cmidrule(r){6-9}\cmidrule{10-13} 
              & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Size}} & \multicolumn{1}{c}{\textit{Spars.}} & \multicolumn{1}{c}{\textit{Acc.}} & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Size}} & \multicolumn{1}{c}{\textit{Spars.}} & \multicolumn{1}{c}{\textit{Acc.}} & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Size}} & \multicolumn{1}{c}{\textit{Spars.}} & \multicolumn{1}{c}{\textit{Acc.}} \\
Method & \multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangledown$} &\multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangle$} \\
\midrule


\gnnexpshort{} ($S=1$) & 0.65 & 1.00 & 0.92 & 0.61 & 0.69 & 1.00 & 0.96 & 0.79 & 0.90 & 1.00 & 0.94 & 0.52 \\
\gnnexpshort{} ($S=2$) & 0.59 & 2.00 & 0.85 & 0.54 & 0.51 & 2.00 & 0.92 & 0.78 & 0.85 & 2.00 & 0.91 & 0.40  \\
\gnnexpshort{} ($S=3$) & 0.56 & 3.00 & 0.79 & 0.51 & 0.46 & 3.00 & 0.88 & 0.79 & 0.83 & 3.00 & 0.87 & 0.34 \\
\gnnexpshort{} ($S=4$) & 0.58 & 4.00 & 0.72 & 0.48 & 0.42 & 4.00 & 0.84 & 0.79 & 0.83 & 4.00 & 0.83 & 0.31 \\
\gnnexpshort{} ($S=5$) & 0.57 & 5.00 & 0.66 & 0.46 & 0.40 & 5.00 & 0.80  & 0.79 & 0.81 & 5.00 & 0.81 & 0.27 \\

\midrule
\OurShort{}               & \textbf{0.21}                              & 2.09                     & 0.90                       & \textbf{0.94}                      & \textbf{0.07}                              & 1.47                     & 0.94                       & \textbf{0.96}                      & \textbf{0.39}                              & 2.39                     & 0.99                       & \textbf{0.96}                 \\
\bottomrule
\end{tabular}
%}
\end{table*}






% \begin{table}[h]
% \centering
% \caption{Results comparing our method (denoted \OurShort{}) to \gnnexplainer{}, for varying values of S. \OurShort{} finds S automatically. Below each metric, $\blacktriangledown$ indicates a low value is desirable, while $\blacktriangle$ indicates a high value is desirable.}
% \label{table:results}
% \setlength{\tabcolsep}{4pt}
% %\footnotesize{
% \begin{tabular}{lrr rr rr}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{\synfour{}}                                                                                                                 & \multicolumn{2}{c}{\synfive{}}                                                                                                                   & \multicolumn{2}{c}{\synone{}}                                                                                                                  \\ 
% \cmidrule(r){2-3}\cmidrule(r){4-5}\cmidrule{6-7} 
%               & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Acc.}} & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Acc.}} & \multicolumn{1}{c}{\textit{Fid.}} & \multicolumn{1}{c}{\textit{Acc.}} \\

% % & \multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\downarrow$} &\multicolumn{1}{c}{$\uparrow$} & \multicolumn{1}{c}{$\uparrow$} \\

% Method & \multicolumn{1}{c}{$\blacktriangledown$} & \multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangledown$} & \multicolumn{1}{c}{$\blacktriangle$} & \multicolumn{1}{c}{$\blacktriangledown$} & \multicolumn{1}{c}{$\blacktriangle$} \\
% \midrule


% \gnnexpshort{} ($S=1$) & 0.65  & 0.61 & 0.69 & 0.79 & 0.90 & 0.52 \\
% \gnnexpshort{} ($S=2$) & 0.59  & 0.54 & 0.51 & 0.78 & 0.85 & 0.40  \\
% \gnnexpshort{} ($S=3$) & 0.56  & 0.51 & 0.46 & 0.79 & 0.83 & 0.34 \\
% \gnnexpshort{} ($S=4$) & 0.58  & 0.48 & 0.42 & 0.79 & 0.83 & 0.31 \\
% \gnnexpshort{} ($S=5$) & 0.57  & 0.46 & 0.40  & 0.79 & 0.81 & 0.27 \\

% \midrule
% \OurShort{}               & \textbf{0.21}                                  & \textbf{0.94}                      & \textbf{0.07}                                        & \textbf{0.96}                      & \textbf{0.39}                                          & \textbf{0.96}                 \\
% \bottomrule
% \end{tabular}
% %}
% \end{table}





\al{\textbf{Comparison to GNN-Explainer:}
Table~\ref{table:results-gnnexplainer} shows the results comparing \OurMethod{} to \gnnexplainer{}. We find that \OurMethod{} outperforms \gnnexplainer{} across all three datasets in terms of both \textit{Fidelity} and \textit{Accuracy}, for all tested values of $S$. We cannot compare \textit{Explanation Size} or \textit{Sparsity} fairly since \gnnexplainer{} requires the user to input the value of $S$. }









% Across all three datasets, we observe that \OurMethod{} outperforms \baserand{} in terms of accuracy with a high margin. We observe accuracy levels upwards of 94\% for \OurMethod{}, indicating that it correctly removes edges that are crucial for the initial predictions in the vast majority of cases (see Table~\ref{table:results}). In contrast, the accuracy levels for \baserand{} are stuck between 17\% and 77\%. %indicating that \OurMethod{} produces much more accurate counterfactul examples. 
\textbf{Summary of the results:} 
Evaluating on four distinct metrics for each dataset gives us a more holistic view of the results. 
% Taking a holistic view of the results, 
We find that for all three datasets, \OurMethod{} can generate CF examples for the majority of nodes in the test set, while only removing a small number of edges. For nodes where we know the ground truth (i.e., those in the motifs) we achieve at least 94\% \textit{Accuracy}. 

Although \baserand{} can generate CF examples for every node, they are not very minimal or accurate. 
The latter is also true for \basekeep{} -- in general, it has the worst scores for \textit{Explanation Size}, \textit{Sparsity} and \textit{Accuracy}. 
\gnnexplainer{} performs at a similar level, indicating that although it is a prominent GNN XAI method, it is not well-suited for solving the CF explanation problem. 

\baserm{} is competitive in terms of \textit{Explanation Size}, but it performs poorly in terms of \textit{Fidelity} for the \synfour{} and \synfive{} datasets, and its \textit{Accuracy} on these datasets is unknown since it is unable to generate \emph{any} CF examples for nodes in the motifs. 
These results show that our method is simple and extremely effective in solving the CF explanation task, unlike existing GNN XAI methods. 
% However, it should be noted that it has higher \textit{Coverage} and \textit{Accuracy} than \OurMethod{} for the \synone{} dataset. 
















